Shelf-Supervised Mesh Prediction in the Wild

We aim to infer 3D shape and pose of object from a single image and propose a learning-based approach that can train from unstructured image collections, supervised by only segmentation outputs from off-the-shelf recognition systems (i.e. 'shelf-supervised'). We first infer a volumetric representation in a canonical frame, along with the camera pose. We enforce the representation geometrically consistent with both appearance and masks, and also that the synthesized novel views are indistinguishable from image collections. The coarse volumetric prediction is then converted to a mesh-based representation, which is further refined in the predicted camera frame. These two steps allow both shape-pose factorization from image collections and per-instance reconstruction in finer details. We examine the method on both synthetic and real-world datasets and demonstrate its scalability on 50 categories in the wild, an order of magnitude more classes than existing works.

==> 3_2_mesh_refine.tex <==
\subsection{Instance-Level Specialization}
\label{sec:method:mesh}
The volumetric representation captures general category-level structure to hallucinate a full 3D shape. However, this shape is coarse as it is: a) limited by the volumetric resolution, and b) generated only from a low-dimensional latent variable. On the other hand, a mesh representation is more flexible and can allow capturing the finer shape details. We therefore go beyond this coarse volumetric prediction, and capture details specific to this instance by converting the volume to an initial mesh, which is then adjusted to better match the input image.


Specifically, our goal is to generate a textured triangle mesh given the segmented input image, the predicted coarse volumetric representation, and the corresponding pose.  We recover an initial mesh from the predicted volumetric occupancy and then  associate each vertex with a feature sampled from both image and volumetric representation.  The vertex locations and features are then iteratively updated to better match the details of the specific input image. 

\textbf{Initialization. } 
Let us denote the mesh as $G = \langle X, T, E\rangle$ where $X$ is the vertex location in space, $T$ the texture or feature associated with each vertex, $E$ the mesh edges. We initialize the mesh geometry $\langle X^0, E^0 \rangle$ from volumetric representation. Following the approach by Mesh-RCNN \cite{gkioxari2019mesh}, we do so by binarizing the occupancy grid $S_o$ and extracting its surfaces. % Every cubic cell  within the surface is converted to a eight vertices, eighteen edges, twelve triangle faces mesh. Then the interior and shared edges and faces are removed, following Mesh-RCNN \cite{gkioxari2019mesh}. %This operation follows operation in Mesh-RCNN \cite{gkioxari2019mesh} and can be processed in batch. 
% The mesh vertices location $X_i$ are obtained from linear interpolating the original volume space bounds ranging from $[-1, 1]$. Note that $X$ are in the canonical frame. Then the mesh samples features from voxel $S_f$ and image $I$ and adjusts its vertex location iteratively, depicted in the next two sections.


% Denote this initial mesh as $M^0 = \langle X^0, E\rangle$ where $E$ denotes edges. 
% However, the volumetric representation is not only memory consuming but also very coarse since it is decoded from a low-dimension latent variable. In this stage, we first convert the volume to a mesh so as to achieve higher resolution and then refine to align it with the input in the predicted view space so as to add on details. 
%  Given a mesh with vertex location $X^k$ at the $k$-th step, 
\textbf{Mesh feature sampling. } Given the initial vertex locations, we associate each vertex with a corresponding global and local feature.
% Specifically, each vertex is associated with a global feature sampled from volumetric representation $S_f$ and a local feature sampled from image.
%The local feature align the predicted mesh with the input image while the global feature provides cues at category-level for the invisible vertices in the input. 
Specifically, for a vertex $X_i$, we associate a global feature via sampling the predicted volumetric feature at the corresponding location: $S_f[X_i]$. 
For every vertex visible in the current view, we also obtain a local feature by sampling an encoding of the images at the location where the vertex is projected, \ie $I_f[\pi(X_i, v)]$. The per-vertex feature for each visible vertex is then initialized as the average of the global and local  sampled features. % (and just global feature for occluded vertices).
% To find the visible vertex in the input image, we find the closest vertex to each pixel from the predicted view.  This process could be performed fast by a rasterizer. The local feature of invisible vertices are set to zeros, i.e. $ w_i I[\pi(X_i, v)]$. 
% Additionally, we leverage the symmetric assumption. For each vertex $i$, we find its nearest symmetric twin $-i$. The symmetric axis is defined in the previous section. If an invisible vertex has a visible twin, it copies the twin's local feature and marks itself as visible. If both are visible, we take the average of the local features. Formally, $$\frac{w_i I[\pi(X_i, v)] + w_{-i} I[\pi(X_{-i}, v)]}{w_i + w_{-i} + \epsilon }, w_i = w_i \lor w_{-i}$$
% To get the final vertex feature, we fuse the global feature with local feature if the vertex is visible.  Formally, we take the weighted average by visibility: $$T_i = \frac{S_f[X_i] + w_i I[\pi(X_i, v)]}{1 + w_i} $$

\textbf{Mesh refinement.}
Given an input mesh, we learn a mesh refinement network $\psi$ takes in a mesh with associated feature $G^k = \langle  X^k, T^k ,E\rangle$ and outputs the displacement of each vertices $\delta X^k$.  In our method, this refinement is performed via a graph neural network \cite{kipf2016semi}.  We repeat this refinement process for certain iterations while resampling the vertex features given the adjusted location $X^{k+1} = X^k + \delta X^k$.
% Specifically,
% $
% \Delta x_i = \psi((x_i,g_i, l_i), POOL\{(x_j, g_j, l_j)\}_{j\in \mathcal{N}(i)})
% $

\textbf{Rendering and Training. }
To supervise the refinement network, we project and render the mesh with feature $G^k$ using a neural renderer $\pi_G$. First, we learn a texture generator that transform the feature $T^k$ to texture for each vertex. Then the textured meshes are rendered to masks and images from the predicted view by a mesh-based differential renderer~\cite{liu2019soft}. The rendered images and masks $(\hat I, \hat M) \equiv \pi_G(G^k, v)$ are encouraged to be consistent with the input image $ \mathcal L_{rgb} = \|\hat I -I\|_1$ and foreground mask $\mathcal L_{mask} = 1 - \frac{\|\hat M\otimes M\|_1}{\|\hat M \oplus M - \hat M \otimes M\|_1};$
% $$
% \mathcal L = \sum_{k=1}^K\|\pi_G(G^k, v) - (I, M)\|_1
% $$
We set $K$ to 5 in our experiments. To further regularize our network, we also add a penalty for large displacement $\|\delta X^k\|_2^2$ and encourage Laplacian smoothness $\|\Delta X^k\|_2^2$.



==> 3_method_gcn.tex <==
\vspace{-2mm}
Our goal is to output a 3D shape in the form of a triangle mesh with texture and the corresponding camera pose. In particular, we are interested in learning this inference in an unsupervised setting, where only images and foreground masks are available as supervision. Towards learning using these image collections as supervision, our insight is that the 3D reconstruction can be learned by enforcing  category-level and instance-level consistency. 

To operationalize this idea, 
we first predict a canonical-frame volumetric representation and a camera pose to capture the coarse category-level 3D structure. 
We then convert this coarse volume to a memory efficient mesh representation which is specialized according to instance-level details. 
% (Section \ref{sec:method:mesh})(Section \ref{sec:method:vol})
% followed by mesh specialization at  instance-level. From the volumetric prediction, we aim to capture the general category-level structure from the data and predict a categorical volumetric representation with the camera pose (Section \ref{sec:method:vol}). 
% In the following specialization process, our goal is to refine the predicted shape in instance-level details by converting the memory inefficient volumetric representation to a mesh and enforcing the consistency with its input image (Section \ref{sec:method:mesh}).
% with to predict a categorical followed by a refinement stage $\psi$ which converts the volume to a mesh $M$ and adjust its shape by enforcing consistency with the input image, shown in Figure \ref{fig:method_overview}. 
% Formally, the shape-pose factorization takes input as foreground image $I$ and outputs a volumetric representation $S$ with camera pose $v$, i.e. $(S, v)\equiv \phi(I)$. In the refinement stage,  a mesh-based representation $G=\langle X, E \rangle$ is constructed by sampling feature from both image $I$ and the volumetric representation $S$. Then, the mesh $G$ is adjusted by the refiner $\psi$, i.e. $\Delta G \equiv \psi(G)$. The sampling and adjusting repeat iteratively. 
To obtain supervision from only image collections, our insight is that the projection of the predicted 3D  should explain the observed images and masks, while also appearing realistic from a novel view. %Specifically, the 3D representation is projected to foreground images and masks by neural render.
% When it is projected from the predicted view, the image should look similar to the input while when it is projected from a novel view, the projection should look realistic. 
% We do not require categorical template, multi-view association, key-points or semantics annotation, known pose,  etc.
% The projection of volume or mesh is realized by neural renders, introduced below. 
% the predicted 3D shapes are projected to images via a volumetric-based or mesh-based  neural renderer $\pi_S, \pi_M $. In addition, a discriminator $\mathcal{D}$ is needed to criticize the rendered views. In the remaining section, we will introduce the concrete form of 3D representation $S, M$ with their conversion, the architecture $\phi, \psi, \pi_{S,M}$, and how to supervise them in details. 

In the Section \ref{sec:method:vol}, we introduce the pursued semi-implicit volumetric representation and our approach to learn unsupervised inference. In Section \ref{sec:method:mesh}, we then examine how we can extract a mesh based representation from our coarse 3D estimate, and subsequently refine it to capture the instance details. 
 
\input{fig/stage1}

\vspace{-3mm}
\subsection{Category-Specific Volumetric Reconstruction}
\label{sec:method:vol}
\vspace{-2mm}
Given an image, we first predict a volumetric representation in a canonical frame with corresponding camera pose. Note that unlike approaches that use a deformable category-level shape space, a volumetric representation allows us to capture larger shape and topology variations.
%The representation aims to capture the coarse shape in the data. The volume-based representation has shown great potential to this end with the ability to handle arbitrary shape and topology \cite{nguyen2019hologan, gadelha2017prgan, lombardi2019neural} and comes as a natural candidate as it is computationally compatible with learning framework\cite{maturana2015voxnet, wu2016learning}. 
Concretely, we adopt a semi-implicit representation comprised of an explicit occupancy grid $S_o$, with an implicit 3D feature $S_f$, i.e. $S=(S_o, S_f)$. The latter can help capture appearance, texture, material, lighting, etc. This allows synthesizing both mask and appearance from a query view, and thereby lets us use both RGB images and foreground masks as supervision. The overall method is depicted in Figure \ref{fig:vol}.

\textbf{Encoder-Decoder Architecture.} We learn a network $\phi$ to predict this semi-implicit representation $(S, v) \equiv \phi(I)$ where $v$ is the camera pose.  The network follows an encoder-decoder architecture with a bottleneck which captures the manifold of shapes within a category. The encoder maps the input image to a low-dimensional latent variable $z$ and predict the camera pose, i.e. $(z, v) \equiv \phi_E(I)$. The latent variable  $z$ is then decoded to the volumetric representation, $S\equiv \phi_D(z)$.
%Note that the decoded shape does not depend on camera pose. 
Empirically, the view-independent decoder learns to predict the shape in a canonical pose across all instances in the category. To further regularize the network, we leverage the observation that many objects exhibit reflectional symmetry, and enforce a fixed symmetric plane ($x=0$) via averaging predicted features and occupancies in symmetrically related locations.

% The two parts are aggregated to render image and masks by the neural renders, $(M, I) \equiv \pi_S(S_f, S_o, v)$. The aggregation follows geometric consistency, introducing a strong inductive bias for shape-pose factorization.  We further argue that the factorziation also benefits from the semi-implicit representation, allowing us to utilize both mask and appearance domains. 
\textbf{Volumetric rendering. } We supervise the 3D prediction using only 2D observations. To this end, we project this semi-implicit volumetric representation to obtain 2D images and masks from a query view i.e. $(I, M) \equiv \pi(S_f, S_o, v)$. Similar to other volumetric neural renderers \cite{lombardi2019neural, drcTulsiani19}, we use a geometrically informed projection process by mimicking ray marching.
%We generate the value of each 2D pixel given a 3D representation and a camera pose.
For each pixel, we shoot a ray from camera through pixel center, and composite samples along the ray to obtain the pixel value. % We follow the previous process to render explicit occupancy to masks. 

%We render the the volumetric feature to obtain a 2D feature in similar manner (Figure \ref{fig:vol} right).
% Consider the feature aggregation process:  $s_f = \pi (S_f, S_o, v)$. 
For a given pixel $\mathbf{p}$, we use $D$ samples  along the ray to obtain a `rendered' feature and mask value. Let us denote the coordinate of the $d$-th sample on the ray as $C_v + \lambda_d e_{\mathbf{p}}$ where  $e_{\mathbf{p}}$ is the corresponding ray direction. We sample both implicit feature and occupancy at these locations, denoted as $S_f[C_v + \lambda_d e_{\mathbf{p}}]$ and  $S_o[C_v + \lambda_d e_{\mathbf{p}}]$. 
% Denote the samples on the ray as $S_f[C_v + \lambda_d e_{ij}]$ that shoots from the camera center $C_v$ to  $i,j$-th pixel center. $e_{ij}$ represents the unit vector of that ray and $S[\cdot]$ represents a bilinear sampling from the feature $S$ given a 3D coordinate. Similarly, denote the ray of samples taken from occupancy as $S_f[C + \lambda_d e_{ij}]$. 
We then composite these samples to obtain a per-pixel feature $s^\mathbf{p}_f$ and mask $s^\mathbf{p}_m$, by using the expected value with respect to ray stopping probability \cite{drcTulsiani17}:
\begin{align*}
% continuous
% f_{ij} &= \int_{\lambda_{near}} ^{\lambda_{far}} p[C+\lambda e_{ij}] S_f[C + \lambda e_{ij}] d\lambda, \\
% p[C+\lambda e_{ij}] &= \int_{\mu_{near}}^{\lambda} 1-S_o[C + \mu e_{ij}]d\mu
% discrete 
s^\mathbf{p}_f = &\sum_{d=1} ^{D} (S_o[C + \lambda_d e_{\mathbf{p}}]  \prod_{h=1}^{d-1} (1-S_o[C + \lambda_h e_{\mathbf{p}}]) ) \\ & \cdot S_f[C + \lambda_h e_{\mathbf{p}}]
% & p[C+\lambda_k e_{ij}] 
\end{align*}
% where $e_{ij}$ represents the unit vector pointing from camera to the center of pixel $ij$. 
The pixelwise mask value $s^\mathbf{p}_m$ is similarly rendered by setting $S_f$ to constant $1$. While this process lets us directly compute the rendered mask $M$, we use a few upconvolutional layers to transform the rendered 2D feature image to the output color image. %  applying a few convolutional layers. % the 2D feature $s_f$ is transformed to shading to obtain RGB images by a $1\times 1$ convolutional layer.   

\textbf{Training.}  
We supervise this network with only unannotated images and foreground masks. We operationalize the following three insights in the loss function. 
% First, the predicted shape and pose should  explain the observed 2D projections. Second, the predicted shape should look plausible from a novel view -- indistinguishable from image collection. Third, the encoder and decoder should be self-consistent. Given an synthesized image from decoder, the encoder should predict the content $(z,v)$ that generates that image.

% \textit{Pixel consistency loss. } First, a plausible predicted shape and pose should  explain the 2D observation. Specifically, we enforce consistency between the projected reconstruction and images with masks. This is performed in pixel space and perceptual space. 
% $$ \mathcal L_{pixel} = \|\pi (S, v)-(I,M)\|_1; ~~~~~~\mathcal L_{perc} = \|h(\pi (S, v))-h(I)\|_1$$
% $h$ is the feature extracted by the discriminators introduced below. 

\textit{Pixel consistency loss. } First, a plausible predicted shape and pose should  explain the 2D observation. Specifically, we enforce consistency between the projected reconstruction and images with masks. This is performed in color space, mask space \cite{liu2019soft}, and perceptual space \cite{zhang2018perceptual}. 
\begin{align*}
    \mathcal L_{rgb} &= \|\hat I -I\|_1 \\
    \mathcal L_{mask} &= 1 - \frac{\|\hat M\otimes M\|_1}{\|\hat M \oplus M - \hat M \otimes M\|_1} \\ 
    \mathcal L_{perc} &= \|h(\hat I)-h(I)\|_2^2
\end{align*}
%  $$ \mathcal L_{rgb} = \|\hat I -I\|_1; ~~~~~~ \mathcal L_{mask} = 1 - \frac{\|\hat M\otimes M\|_1}{\|\hat M \oplus M - \hat M \otimes M\|_1}; ~~~~~~\mathcal L_{perc} = \|h(\hat I)-h(I)\|_2^2$$
where $\hat I, \hat M$ are rendered image and mask; $h$ is the feature extracted by a pretrained AlexNet \cite{krizhevsky2012imagenet} and $\oplus \otimes$ are element-wise summation and production respectively.


\textit{View synthesis adversarial loss. } A degenerate solution could arise such that the shape is only plausible from the predicted view. 
To avoid it, we require the projection of predicted shape to appear realistic from a random novel view.
% look like images in the training set. the predicted shape should look plausible from a novel view -- 
Specifically, we sample another camera pose from a fixed prior to render the novel view:  $I' = \pi(\phi_D(z), v'), v'\sim p(v)$. We then present this generated image to an adversarial discriminator with an objective to fool it. We similarly  encourage photo-realism when rendering from the  predicted camera pose. The loss is minimized in a vanilla GAN \cite{goodfellow2014generative} scheme.
$$
L_{adv} = \log \mathcal{D}(I) + \log (1-\mathcal D (\pi(S, v)) + \log (1-\mathcal D (\pi(S, v'))
$$

\textit{Content consistency loss. } To further regularize the network we build on a insight that the encoder and decoder networks should be self-consistent. Given a synthesized image from the decoder, the encoder should predict the actual content that generated that image. 
% To further regularize the network, we enforce that the encoder-decoder to be self-consistent -- the predicted content should be consistent with the actual content to generate the images. 
Formally, 
\begin{align*}
    \mathcal L_{content} = \|\phi_E(\pi_S(S, v))-(z,v) \|_2^2 \\ + \|\phi_E(\pi_S(S, v'))-(z,v')\|_2^2
\end{align*}
Empirically, we found $\mathcal L_{content}$ crucial to stablize training. 

\textbf{Optimization.} The renderer and decoder are trained to minimize all of the above objectives. However, following \cite{larsen2015autoencoding}, the encoder does not optimize the adversarial loss.
%, only allowed to learn the mapping in the latent space, as suggested by VAE-GAN \cite{larsen2015autoencoding}.  

% \todo{put to formally}
% \begin{align*}
% \phi_E &: \min \mathcal{L}_{pixel} + \mathcal{L}_{perc} + \mathcal{L}_{content}  \\
% \phi_D, \pi &: \min \mathcal{L}_{pixel} + \mathcal{L}_{perc} + \mathcal{L}_{content} + \mathcal{L}_{adv} \\
% \mathcal{D} &: \max \mathcal{L}_{adv}
% \end{align*}

% \subsubsection{Architecture details*}
% Style GAN, Batch size, weight, etc. put to supplementary...
\input{fig/stage2}
\subsection{Instance-Level Specialization}
\label{sec:method:mesh}
The volumetric representation captures general category-level structure to hallucinate a full 3D shape. However, this shape is coarse as it is: a) limited by the volumetric resolution, and b) generated only from a low-dimensional latent variable. On the other hand, a mesh representation is more flexible and can allow capturing the finer shape details. We therefore go beyond this coarse volumetric prediction, and capture details specific to this instance by converting the volume to an initial mesh, which is then adjusted to better match the input image.


Specifically, our goal is to generate a textured triangle mesh given the segmented input image, the predicted coarse volumetric representation, and the corresponding pose.  We first recover an initial mesh from the predicted volumetric occupancy and then  associate each vertex with a texture sampled from the image. The vertex locations together with camera pose are then jointly optimized to better match the details of the specific input image. 

\textbf{Initialization. } 
Let us denote the mesh as $G = \langle X, T, E\rangle$ where $X$ is the vertex location in space, $T$ the texture  associated with each vertex, $E$ the mesh edges. We initialize the mesh geometry $\langle X^0, E^0 \rangle$ from volumetric representation. Following the approach by Mesh-RCNN \cite{gkioxari2019mesh}, we do so by binarizing the occupancy grid $S_o$ and extracting its surfaces. % Every cubic cell  within the surface is converted to a eight vertices, eighteen edges, twelve triangle faces mesh. Then the interior and shared edges and faces are removed, following Mesh-RCNN \cite{gkioxari2019mesh}. %This operation follows operation in Mesh-RCNN \cite{gkioxari2019mesh} and can be processed in batch. 

\textbf{Mesh texture sampling. } Given the vertex locations, we associate each vertex with a corresponding texture from the input image. 
Specifically, for every vertex, we first obtain its visibility together with its texture by sampling the pixel of the images at the location where the vertex is projected, \ie $w_i\in\{0, 1\}; \hat t_i = I[\pi(X_i, v)]$. Furthermore, we leverage the symmetry of the mesh to fuse the textures from its reflective symmetric vertex. The final associated texture for each vertex is an average of itself and its symmetric neighbors, \ie $t_i = \frac{w_i \hat t_i + w_{S(i)} \hat t_{S(i)}}{w_i + w_{S(i)} + \epsilon }$, where $S(i)$ indexes the nearest neighbor of vertex $i$ in the symmetric mesh. 

% For vertex invisible from the current view,  The per-vertex feature for each visible vertex is then initialized as the average of the global and local  sampled features. % (and just global feature for occluded vertices).
% To find the visible vertex in the input image, we find the closest vertex to each pixel from the predicted view.  This process could be performed fast by a rasterizer. The local feature of invisible vertices are set to zeros, i.e. $ w_i I[\pi(X_i, v)]$. 
% Additionally, we leverage the symmetric assumption. For each vertex $i$, we find its nearest symmetric twin $-i$. The symmetric axis is defined in the previous section. If an invisible vertex has a visible twin, it copies the twin's local feature and marks itself as visible. If both are visible, we take the average of the local features. Formally, $$\frac{w_i I[\pi(X_i, v)] + w_{-i} I[\pi(X_{-i}, v)]}{w_i + w_{-i} + \epsilon }, w_i = w_i \lor w_{-i}$$
% To get the final vertex feature, we fuse the global feature with local feature if the vertex is visible.  Formally, we take the weighted average by visibility: $$T_i = \frac{S_f[X_i] + w_i I[\pi(X_i, v)]}{1 + w_i} $$

\textbf{Mesh refinement. }
To specialize the mesh with respect to the input, we optimize the geometry and refine the texture of the mesh iteratively. Given a posed textured input mesh 
% $(v^k, G^k = \langle  X^k, T^k ,E\rangle)$
, we first optimize the vertex location and the camera pose such that the projection of the mesh matches the observation. After every updates of mesh geometry, vertex textures are re-sampled from the image given the adjusted projected location. % $X^{k+1} = X^k + \delta X^k$. 


To project and render the mesh with texture we use a neural renderer $\pi_G$. The textured meshes are rendered to masks and images from the predicted view by a mesh-based differential renderer \cite{liu2019soft}. The rendered images and masks $(\hat I, \hat M) \equiv \pi_G(G, v)$ are encouraged to be consistent with the input image $ \mathcal L_{rgb} = \|\hat I -I\|_1$ and foreground mask $\mathcal L_{mask} = 1 - \frac{\|\hat M\otimes M\|_1}{\|\hat M \oplus M - \hat M \otimes M\|_1}$. We regularize the optimization by penalizing large vertex displacement  $\|\delta X\|_2^2$ and encourage Laplacian smoothness $\|\Delta X^k\|_2^2$. 

% The  update of mesh geometry and texture sampling are repeated iteratively for every optimization step.
% Every optimization step outputs the displacement of each vertices and camera pose.  
% learn a mesh refinement network $\psi$ takes in a mesh with associated feature $G^k = \langle  X^k, T^k ,E\rangle$ and outputs the displacement of each vertices $\delta X^k$.  In our method, this refinement is performed via a graph neural network \cite{kipf2016semi}.  We repeat this refinement process for certain iterations while resampling the vertex features given the adjusted location $X^{k+1} = X^k + \delta X^k$, and 
% Specifically,
% $
% \Delta x_i = \psi((x_i,g_i, l_i), POOL\{(x_j, g_j, l_j)\}_{j\in \mathcal{N}(i)})
% $

% To supervise the refinement network, we project and render the mesh with feature $G^k$ using a neural renderer $\pi_G$. First, we learn a texture generator that transform the feature $T^k$ to texture for each vertex. Then the textured meshes are rendered to masks and images from the predicted view by a mesh-based differential renderer~\cite{liu2019soft}. 
% $$
% \mathcal L = \sum_{k=1}^K\|\pi_G(G^k, v) - (I, M)\|_1
% $$
% We set $K$ to 5 in our experiments. To further regularize our network, we also add a penalty for large displacement $\|\delta X^k\|_2^2$ and encourage Laplacian smoothness $\|\Delta X^k\|_2^2$.



==> 3_old_method.tex <==
The goal is to learn a model to infer the volumetric 3D structure $V$ given a single image $I$. \todo{ $\to$ replace:} We learn only from a collection of images $\{I_i\}_{i=1:N}$ and silhouette $\{M_i\}_{i=1:N}$. We focus on learning structure from images of the same categories. However, this is an ill-posed problem since multiple 3D structures could induce the exact same 2D projection. 
For example, the model could account shape variance to explain view-point variance. 
Rather than predicting viewer-centric 3D voxels, we estimate 3D canonical pose and view point separately and then transform 

Our model follows encoder-decoder architecture and is trained in the VAE-GAN \cite{vae-gan} fashion. There are three modules: 1) an encoder $\mathbf{E}$ that takes in an image and infers the latent shape code $z$ with estimate view point $v$; a decoder $\mathbf{G}$ that takes in both shape code and view point $z, v$ and generates a view-independent 3D shape $V=\mathbf{G_1}(z)$ and its projected 2D image $\hat I = G_2(V, v)$ given the view point. The generated images are then presented to a 3) discriminator $\mathbf{D}$. The encoder-decoder are jointly optimized such that those images $\{\hat I_i\}$ cannot be differentiated from the real image  distribution $\{I_i\}$. \todo{z0,v2... intuition.}

\subsection{Encoder and View Estimation} 

The first step is to infer latent variable $z$ and viewpoint $v$ from the image. Intuitively, the latent code $z$ encode view-independent information, such as the canonical shape and texture. For camera pose, we assume the camera always points upright, with the same distance from the properly centered objects. Then the camera pose distribution  lives in a $SO(2)$. The viewpoint $v$ represents elevation and azimuth angle of the perspective camera. When we sample a viewpoint, both elevation and azimuth are sampled from a uniform distribution independently.  The encoder is implemented by a simple convolutional neural network with two heads to predict $z$ and $v$, respectively.
 

\subsection{Decoder}
The decoder takes input as a latent code $z$ and viewpoint $v$, which are either from encoder or sampling. It outputs the explicit 3D volumetric representation and the projected images under viewpoint $v$. 
 
\textbf{Feature Projection Module. }
Decoder: Explicit ray marching. Style 


\textbf{Discriminator}
Discriminator: Style Discriminator

Encoder: predict z, view point.


\subsection{Optimization.} 
$$
\min_{G} \max_{D} \mathbb E_x[\log(D(x))] + \mathbb E_{z}\log(1-D(G(z)))
$$

% The images depict different instances from the same category. But multiple views of the same instance are not required. Furthermore, we do not assume any template shape or paired view-point and images labels. 


The underlying 3D shapes and viewpoint estimation emerge from image collections without 3D or viewpoint annotation. To explain the observed images with parsimony, the model should factorize 3D shape from view-point. The 3D shape should capture both the categorical common shape and finer instance details. 

Training : (z0, v2) blah blah blah. sample view 

==> 6_broader_statement.tex <==
The broader impact will be reconstructing 3D for arbitrary images from generic categories. The current challenge is the requirement of supervision in many forms, such as expensive 3D ground-truth, pose annotations, etc.  Our work takes a step to relax the requirement especially when foreground masks could even be obtained automatically. 

In terms of  application, it could be used in augmented reality or virtual reality (AR/VR). Instead of wearing a VR helmet, the user could just hold a monocular device such as a mobile phone, a laptop camera to record scenes around him/her and lift them into 3D. The positive impact will be making 3D content creation easier for people without a technical background. It also has the potential to transform communication routines among people, bringing people closer regardless of geographical distance.  However, a common concern is producing biased reconstruction hidden in the training  data. Our instance-specific specialization could reduce the possibility to predict such a bias among data in categories. However, further extensive works are needed before conclusive statement.

==> exp/open_image.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{exp/canvas_bg50_med_16x3.png}
    \caption{Caption \todo{update.}}
    \label{fig:my_label}
\end{figure*}

==> exp/progress.tex <==
\begin{figure*}
    \vspace{-3mm}
    \centering
    \includegraphics[width=\linewidth]{exp/real_chair_long.png}
    % \includegraphics[width=0.25\linewidth]{exp/progress.png}
    \caption{Left: visualizing reconstructed shapes and texture of chairs in the wild from a novel pose and the predicted pose. Right: projected mesh after every step of instance-level specialization. }
    \label{fig:progress}
\end{figure*}

==> exp/quant_mesh.tex <==
\begin{table}[t]
    \caption{\todo{judy: cut F score. }Quantitative results on ShapeNet comparing with and without instance-level specialization. }
    \centering
    \footnotesize
    % \begin{tabular}{m{2cm}| m{0.6cm}m{0.6cm}m{0.6cm}| m{0.6cm}m{0.6cm}m{0.6cm}|m{0.6cm}m{0.6cm}m{0.6cm} }
    \begin{tabular}{r  ccc  ccc  ccc }
\toprule
&  \multicolumn{3}{c}{Aero} & \multicolumn{3}{c}{Car} & \multicolumn{3}{c}{Chair} \\
& F@5\% & F@2\% & F@1\% & F@5\% & F@2\% & F@1\% & F@5\% & F@2\% & F@1\% \\
\midrule
Initial & 0.78 &	0.32 &	0.14 &	 0.63 &	0.25 &	0.10	& 0.58 &	0.25  &	0.10\\
Refined & 0.85 &	0.55 &	0.31 &	 0.63 &	0.32 &	0.14	& 0.60 &	0.28 &	0.13\\
% \hline
% Refined template & 0.87 &	0.58 &	0.32 &	 0.66 &	0.33 &	0.15	& 0.60 &	0.27 &	0.12\\
\bottomrule
\vspace{-7mm}
\end{tabular}
    \label{tab:my_label}
\end{table}

==> exp/rebuttal.tex <==

\begin{figure}[b]
\vspace{-3mm}
\begin{floatrow}
% \MyBox{
\ffigbox[10cm]{%
  \includegraphics[width=.9\linewidth]{exp/ablation.png}
}{%
  \caption{Ablation: the 1st row visualizes the reconstructed shape from the predicted view. The 2nd row shows the shape from a novel view.}%
    \label{fig:ablation}
}

\capbtabbox{%
    \begin{tabular}{cccc}
    \toprule
     & aero & car & chair \\
     \midrule
Ours & 0.45 & 0.59 &	0.31 \\
Ours  $-\mathcal L_{adv}$ & 0.25 & 0.44 & 0.22 \\
Ours $-\mathcal L_{cont}$ & 0.24 & 0.54 & 0.23 \\
% Ours $-\mathcal L_{cont} + \mathcal L_{pose}$  & 0.35 & 0.57 & 0.31 \\
\bottomrule
    \end{tabular}
}{    
    \caption{Quantitative results on ShapeNet to ablate the effect of each loss term. }
    \label{tab:ablation}
}
\end{floatrow}
\end{figure}


==> exp/refine_ablation.tex <==
\begin{figure}
    \centering
    \includegraphics[width=.7\linewidth]{exp/ablation_init.png}
    \caption{Ablation study to visualize the refined mesh initialized from another template whose shape is far from the ground-truth shape.}
    \label{fig:ablation_init}
\end{figure}

==> exp/vis_quads.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{exp/vis_quads.png}
    \caption{Visualizing reconstructed shapes on quadrupeds from a novel pose (2nd-3rd row) and the predicted pose (last row). }
    \label{fig:vis_quads}
\end{figure}

==> ext/rebuttal.tex <==
https://docs.google.com/spreadsheets/d/1rpDKfF60-8PaRZqcSDpj1rQfsLezzDs469bA3etoRhI/edit?usp=sharing
